Impact of Human-AI Interaction on User Trust and Reliance in AI-Assisted Qualitative Coding

While AI shows promise for enhancing the efficiency of qualitative analysis, the unique human-AI interaction resulting from varied coding strategies makes it challenging to develop a trustworthy AI-assisted qualitative coding system (AIQCs) that supports coding tasks effectively. We bridge this gap by exploring the impact of varying coding strategies on user trust and reliance on AI. We conducted a mixed-methods split-plot 3x3 study, involving 30 participants, and a follow-up study with 6 participants, exploring varying text selection and code length in the use of our AIQCs system for qualitative analysis. Our results indicate that qualitative open coding should be conceptualized as a series of distinct subtasks, each with differing levels of complexity, and therefore, should be given tailored design considerations. We further observed a discrepancy between perceived and behavioral measures, and emphasized the potential challenges of under- and over-reliance on AIQCs systems. Additional design implications were also proposed for consideration.

==> others.tex <==
\subsection{Independent Variables}
\begin{table}[htbp]
\begin{tabular}{@{}llll@{}}
\toprule
\multirow{2}{*}{\begin{tabular}[c]{@{}l@{}}Number of Top K \\ Suggestions\end{tabular}} & \multicolumn{3}{c}{Model Performance} \\ \cmidrule(l){2-4} 
 & Natural Model & Perfect Model & Random Model \\ \midrule
No suggestions but with codebook& / & / & / \\ \cmidrule(r){1-1}
1 suggestions+view more &  &  &  \\ \cmidrule(r){1-1}
5 suggestions+view more &  &  &  \\ \cmidrule(r){1-1}
All suggestions &  &  &  \\ \bottomrule
\end{tabular}
\end{table}


\subsection{Alternatives}

Top1 + show more.

Top5 + show more.

A codebook.


\begin{figure}[htbp]
  \centering
  \includegraphics[width=0.5\linewidth]{figure/Behaviors.png}
  \caption{User Behaviors along the Qualitative Coding Process}
\end{figure}


\subsection{Ambiguity}
Ambiguity Decrease: state code levels, dataset introduction, desired codes examples, desired contents (opinions and attitudes), how will the model perform better, definitions about initial codes. 

Normal Ambiguity.

\subsection{Metrics}
\subsubsection{Homogeneity}
\subsubsection{Cosine Similarity}
\subsubsection{Purity}


% \subsection{Code Start Problem}
% There are two types of cold start problems: product cold start and user cold start. An expert user could be familiar with coding but not familiar with the model. Thus he/she needs to spend much time to explore systems. A novice could not be familiar with coding but also not familiar the model. This issue is especially important because a user who receives poor-quality recommendations may opt to left the system before giving enough interaction to allow the recommender to understand his or her interests. 

% There are several strategies to help users to start from scratch. One is to use pre-defined codes. 

% However, too many pre-defined codes could limit users' creativity and are not aligned with the rule that users should think freely and propose their own codes during open coding process. But if we don't provide some pre-defined codes for users. Some people, especially novices, could not learn from these codes and thus cannot start. However, they could over rely on these codes. And thus not propose new codes. But for experts, they may prefer to propose codes by themselves. 

% Thus we propose a research question: 

% \textbf{RQ3: How will expert coder and novices coder react to different amount initial codes? There is also discussion on learnable codes. If models are not learnable, that is, fixed prediction suggstions, how will novices and experts react?}



% \section{Study2: Code Start Problem}

% At the end of each session, we let users fill up survey and understand their trust to code suggestions to observe the change of their trust to code suggestions. 

% Users were then invited to use CoAIcoder with enhanced explainable functions.

% \subsection{Experiment Conditions}
% \begin{enumerate}
%     \item Users \{ Expert, Novice \}
%     % \item Alternatives \{1+show more, 5+show more, All \}
%     \item Initial Codes \{ Pre-defined codes, No pre-defined \}
% \end{enumerate}

% \begin{table}[htbp]
% \begin{tabular}{@{}cll@{}}
% \toprule
%  & \multicolumn{1}{c}{\textbf{Expert (E)}} & \multicolumn{1}{c}{\textbf{Novice (N)}} \\ \midrule
% \textbf{Pre-defined codes (P)} & P\_E & P\_N \\
% \textbf{No pre-defined (N)} & N\_E & N\_N \\ \bottomrule
% \end{tabular}
% \end{table}

% \section{Study3: Number of TopK suggestions}
% \begin{enumerate}
%     \item Number of TopK suggestions \{ 5+show more, Show all suggestions, Show codebook but no suggestions \}
% \end{enumerate}



% Consequently, this work aims to further understand how to build trustworthy AI-assisted qualitative coding tool, with a focus on studying the influence of two factors: ambiguity and controllability. 


% An important purpose in HCI and AI area is to build a system that worth trust from users. It is well known that AI's capabilities are based on statistics and probabilities and the user should not fully trust the system, it will be good if an AI system can behave trustworthy because users 
% would like to use or rely on the product more in a long run \cite{GoogleAI}.

% Building trustworthy AI applications or models requires a lot of effort, especially for qualitative analysis, which is flagged as 


% Therefore, many people take a cautious stance on applying AI to support qualitative coding \cite{jiang2021supporting}. Some pessimistic people believe that AI cannot assist, and even optimistic people do not want AI to "do it all" for them either, thus relinquishing their control over data because the new discoveries they made through their research process are the most valuable \cite{jiang2021supporting, rietz2021cody}. Additionally, they would like to see some learning ability of AI algorithms as the emergence of new codes rather than relying on predefined categories \cite{jiang2021supporting, chen2018using}. Rietz et al. also think that the system should provide multiple codes instead of just one code to improve fault tolerance \cite{rietz2021cody}.

% Three major AI methods are used to do qualitative analysis: keywords and rule-based query \cite{marathe2018semi, kaufmann2020supporting, rietz2021cody}, topic modeling \cite{leeson2019natural, baumer2017comparing, bakharia2016interactive, lennon2021developing} and text classification \cite{rietz2021cody}.


%add more trust things (simplely)
%like transparency, explanations
%how to improve transparency, but not focus on ambiguity.

% Applying AI in qualitative coding is quite unique. A typical AI model lifecycle includes four phases: data collection, organization, model building and model employing \cite{fischer2020ai, haakman2021ai}. After that, a relatively mature model can be used to apply a trained model to do classification or prediction. On the contrary, qualitative analysis requires \textit{end users} to propose classes in the open coding process, and then train a model for their rest coding process while the normal system usually generate model and classes by the developers. A data generator is also a data trainer and consumer at the same time. 


% Particularly, some users could have a very long or specific code, caused over-fitting problem (fitting aspects of data that are not generalizable outside the data), while sometimes providing a broad phrase, caused underfitting problems. Either situation will be harmful to the training of good models. In fact, the nature of ambiguity, lack of correct answers, and relying on human creativity caused that people have low trust to AI's ability to reliably predict codes \cite{jiang2021supporting, chen2018using, drouhard2017aeonium}.

% There are four main different ambiguity in natural language, lexical ambiguity, syntactic, (structural) ambiguity, semantic ambiguity and pragmatic ambiguity \cite{ceccato2004ambiguity}.





%\subsection{Stakeholders and System Development cycle}

% \section{Preliminary Study}
% We observed that different users have different accepted rate on the same materials and system. Some have higher

% \section{Formative Study}
% We invited 5 users to participate a longitudinal study.

% RQ1: Will users' accepted rate become stable after a period usage if using our system?

% RQ2: How many suggestions we should provide?

% RQ3: Will users adopt different granularity when do coding?

% RQ4: Do users believe our systems' ability?





==> paper/6.1_results_rq1_v1.tex <==
\subsection{RQ1: Impact on \added{Model Performance} \deleted{Code Prediction Relevance}}
\label{sec:RQ:code-relevance}

\added{The performance of the model for both automatic and human evaluation is reported in Table \ref{tab:model_performance}.}

\begin{table}[htbp]
\caption{\added{The model's performance was evaluated through both automatic and human assessments. Note that the recall@5 metric was only available in the automatic evaluation.}}
\label{tab:model_performance}
\scalebox{0.85}{\begin{tabular}{|c|c|ccc|cc|}
\hline
\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Factor1: \\ Code Granularity\end{tabular}}} & \multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Factor2: \\ Text Granularity\end{tabular}}} & \multicolumn{3}{c|}{\textbf{Automatic Evaluation}} & \multicolumn{2}{c|}{\textbf{Human Evaluation}} \\ \cline{3-7} 
 &  & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Precision@5\\ (M ± S.D.)\end{tabular}} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Recall@5\\ (M ± S.D.)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}MAP@5\\ (M ± S.D.)\end{tabular} & \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Precision@5\\ (M ± S.D.)\end{tabular}} & \begin{tabular}[c]{@{}c@{}}MAP@5\\ (M ± S.D.)\end{tabular} \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Short Codes \\ (1-3 words)\end{tabular}} & Sentence & \multicolumn{1}{c|}{0.16 ± 0.18} & \multicolumn{1}{c|}{0.30 ± 0.39} & 0.47 ± 0.13 & \multicolumn{1}{c|}{0.20 ± 0.09} & 0.38 ± 0.15 \\ \cline{2-7} 
 & Paragraph & \multicolumn{1}{c|}{0.20 ± 0.13} & \multicolumn{1}{c|}{0.68 ± 0.41} & 0.68 ± 0.23 & \multicolumn{1}{c|}{0.21 ± 0.13} & 0.53 ± 0.31 \\ \cline{2-7} 
 & Selective & \multicolumn{1}{c|}{0.20 ± 0.16} & \multicolumn{1}{c|}{0.47 ± 0.45} & 0.53 ± 0.12 & \multicolumn{1}{c|}{0.21 ± 0.11} & 0.43 ± 0.19 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Long Codes \\ (4-6 words)\end{tabular}} & Sentence & \multicolumn{1}{c|}{0.16 ± 0.20} & \multicolumn{1}{c|}{0.18 ± 0.19} & 0.42 ± 0.14 & \multicolumn{1}{c|}{0.17 ± 0.08} & 0.37 ± 0.16 \\ \cline{2-7} 
 & Paragraph & \multicolumn{1}{c|}{0.54 ± 0.24} & \multicolumn{1}{c|}{0.65 ± 0.20} & 0.72 ± 0.23 & \multicolumn{1}{c|}{0.44 ± 0.15} & 0.80 ± 0.16 \\ \cline{2-7} 
 & Selective & \multicolumn{1}{c|}{0.42 ± 0.35} & \multicolumn{1}{c|}{0.34 ± 0.29} & 0.57 ± 0.23 & \multicolumn{1}{c|}{0.35 ± 0.24} & 0.56 ± 0.26 \\ \hline
\multirow{3}{*}{\begin{tabular}[c]{@{}c@{}}Mixed Codes \\ (1-6 words)\end{tabular}} & Sentence & \multicolumn{1}{c|}{0.08 ± 0.10} & \multicolumn{1}{c|}{0.20 ± 0.31} & 0.32 ± 0.09 & \multicolumn{1}{c|}{0.12 ± 0.03} & 0.44 ± 0.11 \\ \cline{2-7} 
 & Paragraph & \multicolumn{1}{c|}{0.54 ± 0.30} & \multicolumn{1}{c|}{0.66 ± 0.20} & 0.62 ± 0.24 & \multicolumn{1}{c|}{0.21 ± 0.07} & 0.76 ± 0.20 \\ \cline{2-7} 
 & Selective & \multicolumn{1}{c|}{0.34 ± 0.22} & \multicolumn{1}{c|}{0.44 ± 0.25} & 0.41 ± 0.11 & \multicolumn{1}{c|}{0.15 ± 0.06} & 0.52 ± 0.11 \\ \hline
\end{tabular}}
\end{table}


\subsubsection{\added{Automatic Evaluation: Precision@5.}}

\added{\codeG. A mixed ANOVA test revealed a significant main effect of \codeG on Precision@5, $F_{(2, 27)} = 3.61$, $p = 0.041$. Pairwise t-test results indicated that the \sh condition ($M = 0.19, SD = 0.16$) had significantly lower precision@5 compared to \mi ($M = 0.32, SD = 0.22$), with $t_{18} = -2.25$, $p = 0.037$, and significantly lower precision@5 compared to \lo ($M = 0.37, SD = 0.28$), with $t_{18} = -2.58$, $p = 0.019$. No significant difference was observed between \lo and \mi.}

\added{\textG. A significant main effect of \textG on Precision@5 was observed, $F_{(2, 54)} = 15.68$, $p < 0.001$. Pairwise t-test results indicated that \sent ($M = 0.13, SD = 0.16$) had significantly lower precision@5 than \sele ($M = 0.32, SD = 0.26$), with $t_{29} = -3.56$, $p < .01 $, and significantly lower precision@5 compared to \para ($M = 0.43, SD = 0.23$), with $t_{29} = -4.38$, $p < .001$. Additionally, \sele ($M = 0.32, SD = 0.26$) demonstrated significantly lower precision@5 compared to \para ($M = 0.43, SD = 0.23$), with $t_{29} = -2.20$, $p = 0.037$.}

\added{\textit{Interactions.} A mixed ANOVA test revealed a significant interaction effect between the two factors, $F_{(4, 54)} = 3.01$, $p = 0.026$. The interaction effect between \codeG and \textG was found in several comparisons: \lo (\sent vs. \sele: $t_{9} = -4.40$, $p < .01$).
\mi (\para vs. \sent: $t_{9} = 6.23$, $p < 0.001$; \para vs. \sele: $t_{9} = 3.16$, $p = 0.012$; Sentence vs. \sele: $t_{9} = -3.36$, $p < .01$).
\sh (\para vs. \sent: $t_{9} = 2.83$, $p = 0.020$).}


\subsubsection{\added{Automatic Evaluation: Recall@5}}


\added{\codeG. A mixed ANOVA test revealed no significant main effect of \codeG on Recall@5.}

\added{\textG. A mixed ANOVA test revealed a significant main effect of \textG on Recall@5, $F_{(2, 54)} = 14.69$, $p < 0.001$. Pairwise t-test results indicated that \sent ($M = 0.23$, $SD = 0.31$) had lower Recall@5 than \sele ($M = 0.41$, $SD = 0.35$), with $t_{29} = -2.69$, $p = 0.012$, and lower recall than \para ($M = 0.66$, $SD = 0.28$), with $t_{29} = -5.12$, $p < 0.001$. Additionally, \sele ($M = 0.41$, $SD = 0.35$) demonstrated lower recall@5 than \para ($M = 0.66$, $SD = 0.28$), with $t_{29} = -3.14$, $p = 0.004$. This suggests that \sent is associated with lower values compared to both \sele and \para levels.}


\added{\textit{Interactions.} There was no significant interaction between the two factors.}


\subsubsection{\added{Automatic Evaluation: MAP@5}} 
\added{\codeG. A mixed ANOVA test revealed no significant main effect of \codeG on MAP@5.}

\added{\textG. A mixed ANOVA test revealed a significant main effect of \textG on MAP@5, $F_{(2, 54)} = 20.30$, $p < 0.001$. Pairwise t-test results indicated that \sent ($M = 0.40$, $SD = 0.12$) had lower MAP@5 than \sele ($M = 0.50$, $SD = 0.15$), with $t_{29} = 3.41$, $p < .01$, and lower MAP@5 than \para ($M = 0.67$, $SD = 0.23$), with $t_{29} = -3.37$, $p < 0.01$. Additionally, \sele ($M = 0.50$, $SD = 0.15$) demonstrated lower MAP@5 than \para ($M = 0.67$, $SD = 0.23$), with $t_{29} = 6.27$, $p < .001$. This suggests that \sent is associated with lower values compared to both \sele and \para levels.}


\added{\textit{Interactions.} There was no significant interaction between the two factors.}


\subsubsection{\added{Human Evaluation: Precision@5}}
\added{\codeG. A mixed ANOVA test revealed no significant main effect of \codeG on precision@5 in human evaluation.}

\added{\textG. A mixed ANOVA test revealed no significant main effect of \textG on precision@5 in human evaluation.}

\added{\textit{Interactions.} A mixed ANOVA test revealed no significant interaction effect between the two factors.}


\subsubsection{\added{Human Evaluation: MAP@5}} 
\added{\codeG. A mixed ANOVA test revealed no significant main effect of \codeG on MAP@5 in human evaluation.}

\added{\textG. A mixed ANOVA test revealed a significant main effect of \textG on MAP@5, $F_{(2, 54)} = 37.00$, $p < 0.001$. Pairwise t-test results indicated that \sent ($M = 0.16$, $SD = 0.07$) had lower MAP@5 than \sele ($M = 0.24$, $SD = 0.14$), with $t_{29} = -4.03$, $p < .01$, and lower than \para ($M = 0.29$, $SD = 0.12$), with $t_{29} = -7.24$, $p < .001$. Additionally, \sele ($M = 0.24$, $SD = 0.14$) demonstrated lower MAP@5 than \para ($M = 0.29$, $SD = 0.12$), with $t_{29} = 4.55$, $p < .001$. This suggests that \sent is associated with lower values compared to both \sele and \para levels.}


\added{\textit{Interactions.} A mixed ANOVA test revealed a significant interaction effect between the two factors, $F_{(4, 54)} = 2.82$, $p = 0.033$. The interaction effect between \codeG and \textG was found in several comparisons: \lo (\sent vs. \para: $t_{9} = -7.28$, $p < .001$).
\mi (\para vs. \sent: $t_{9} = -5.12$, $p < 0.01$; \para vs. \sele: $t_{9} = 4.46$, $p = 0.014$).}







\deleted{We discuss the \suggestionQuality of the top five code suggestions provided by \name. The code quality score is the average overlap between the considered suggestion and the final code as chosen by the users.
The results are shown in Figure \ref{fig:rq1:accuracy} and the statistical analysis is presented in Appendix Table~\ref{tab:codequality}.}

\deleted{\paragraph{Text Granularity.} Overall, we observed a significant main effect of \textG on \suggestionQuality{} for all Top 5 suggestions (Top1 to Top5), except for Top 2. The quality was higher for the \paraS ($M=0.54$ across 5 suggestions) compared to \sentS ($M=0.19$ across 5 suggestions) and \seleS ($M=0.31$ across 5 suggestions).}

\deleted{\paragraph{Code Granularity.} We observed a main effect of \codeG on \suggestionQuality for all Top 5 suggestions (Top1 to Top5). The \suggestionQuality is lower in the \sh conditions generally ($M=0.23$ across 5 suggestions) compared to \mi ($M=0.39$ across 5 suggestions) and \lo ($M=0.42$ across 5 suggestions).}

\deleted{\paragraph{Specific Conditions.} 
Looking at the \paraS conditions where the \suggestionQuality was the highest, we observe that the \suggestionQuality across different \codeG varies a lot. This is shown by the interactions we observed (Top 3, Top 4). 
The overall highest \suggestionQuality in the \lo $\times$ \para ($M=0.64$ across 5 suggestions) and \mi $\times$ \para  ($M=0.63$ across 5 suggestions), with a remarkably lower performance of \sh $\times$ \paraS ($M=0.25$ across 5 suggestions). We also observed high variances in the \paraS conditions.}


\subsubsection{\added{Summary}}

\added{The model demonstrably surpasses both \sele and \sent, with the exception of \sh $\times$ \para, in both automatic and human evaluations when tasked on \para. This performance enhancement could possibly stem from the more verbose selected text in the \para configuration, providing an enriched data set for the classifier to utilize.
However, the model's efficacy diminishes  when interacting with more succinct codes—\sh underperforms in comparison to \mi and \lo. The rationale for this pattern may be traced back to the differing levels of detail embedded in the codes. Shorter codes inherently convey less information, potentially reducing the likelihood of a match between users' codes and the chosen text. This could result in diminished similarity scores, and consequently, a weaker correlation between the code and text.}



\deleted{Our AI suggestion seemed to have better in the \lo and \mi conditions--even more when meeting \para settings (except \sh $\times$ \para). This comes from the different levels of specificity of the codes: longer codes could contain more information for the text and have a better chance to have relevant meaning with selections; \para usually has more generic codes, making the codes have a higher chance to be relevant with other text.}





==> paper/7_discussion_v1.tex <==
\subsection{Behavior Trust is High with Better Suggestions}
When looking at \emph{Text Granularity}, our results show that for simpler tasks (i.e.  at \sele and \sent levels), \bt is higher, as users tend to use the suggestions more: users selected a suggestion more than 26\% for \sele and \sent, in contrast to 16\% in the \para conditions. Participants reported that the suggestions were less relevant on \para tasks, based both on the reduced data used for training and length of text which makes it hard to summarize a paragraph. 
This issue of creating a suitable code is even stronger in the \sh $\times$ \para conditions which yields the lowest \sr for suggestions. 
Like P8 (\sh $\times$ \para) said, \textit{"I think the recommendation for the first one (short $\times$ sentence). It was still okay, like sometimes the codes was there, sometimes they were not there. But I think for this one (short $\times$ paragraph), there is too little information given/offered to the model. So the model did not really recommend me much."}
So it is fair to assume that users will display a higher level of trust with better suggestions.
\simon{<< Discuss code quality as well >>}
\gao{For harder task, users' are more acceptable for the imperfect code suggestions}

\subsection{But Perceived Trust is High with Harder Tasks}
While we noted that \bt was the lowest for \para settings, we also found out that \pt was overall the highest compared to the other conditions except \sh $\times$ \para. This result is surprising as \bt is clearly lowest under these experimental conditions. When discussing with participants, they reported that the \para tasks were deemed as the hardest, as it is harder to find a label for a code that fits an entire paragraph as opposed to a shorter textual unit (\sele or \sent).
When performing the \para tasks, users would check and refer all the suggestions provided by the AI, and while they reported that the suggestions were individually not good enough to be selected (hence the low \sr), they would still be able to use them to start building their own code. This is validated in user's subject preferences (RQ3). 

\subsection{Managing Trust Expectations and Usefulness of AI}
From our experiment, and given the differences in terms of \bt and \pt we observed, we understand that trust is a complex notion. Previous literature highlighted that trust is correlated with accuracy (or the quality of the suggestions) \cite{papenmeier2022s, yin2019understanding}. Our results confirm this general trend: \bt (through \sr) was generally higher in conditions with better suggestions (\sele and \sent).
However, our observations on \pt for harder tasks, also suggests that the trust we measured depends on users' expectation. In situations where the tasks gets significantly harder to perform, users will appreciate any help, even if not very accurate. As such, our AI system was useful for users for both simple (\sele and \sent) and hard (\para) tasks regardless its accuracy which sheds new light into how AI can be used for qualitative coding. 

\subsection{Text Granularity in Real Life}
\simon{<< Discuss code quality >> briefly}
We considered \emph{Text Granularity} as a factor. By using this factor, we were able to highlight interesting differences between \pt and \bt. All three levels we chose have applications in real life.

\subsubsection{\emph{\sele} is Best for Coding}
\sele coding is closest to how a single coder may start exploring data in real life, and select the most relevant phrases before generating a label. As stated above, the highest levels of \bt were observed in \sele coding.

\subsubsection{\emph{\sent} for Collaborative Coding}
From our analysis of selection behavior (length of selections, number of selections), \sele and \sent coding are overall rather similar, despite some significant differences, as the gap between these two conditions is way lower than the gap between these two and \para.
While \sele should usually be the default granularity for coding, \sent level coding can be useful for collaborative coding, where two users need to reach some level of consistency. In particular, for the computation of inter-rater reliability scores, one may need to choose a simple, unambiguous text selection unit, in which case, sentence level makes more sense.

\subsubsection{\emph{\para} for Summarizing Long Texts}
Finally, the \para task is less likely to be used for qualitative coding in real life. However, the AI system we developed could still be useful for users trying to summarize a long text. In that case, going for a \para helps summarizing entire pages in a few sentences. The low \sr of our system suggest that our AI system should improve the quality of the suggestions. However, as highlighted in the subsections above, the help the system is able to provide will still be greatly appreciated by our participants. 

\gao{\subsection{Mix and Selective Coding is good for AI, while not good for human's perceived reliability}}






==> paper/7_discussion_v2.tex <==

% \gao{To make AI perform better, they can shorten their codes but provide more information for their own usage (like put more information into comment function, and for the system to generate more idea based on this, to show system's ability) \simon{need literature}}

% \subsection{Managing Trust Expectations and Usefulness of AI}
% From our experiment, and given the differences in terms of \bt and \pt we observed, we understand that trust is a complex notion. Previous literature highlighted that trust is correlated with accuracy (or the quality of the suggestions) \cite{papenmeier2022s, yin2019understanding}. \added{Our results show a more nuanced view}: \bt (through \sr) was generally lower in conditions where participants found the suggestions worse (\paraS).
% However, our observations on \pt for harder tasks, also suggests that the trust we measured depends on users' expectation. In situations where the tasks gets significantly harder to perform, users will appreciate any help, even if not very accurate. As such, our AI system was useful for users for both simple (\sele and \sent) and hard (\para) tasks regardless of its accuracy which sheds new light into how AI can be used for qualitative coding.

% \added{Similarly, our results on \cq (where \paraS achieved a higher score) suggests that comparing the quality of the suggestion across different tasks and text granularity could be potentially misleading. Indeed, the coding task in the \paraS conditions was more superficial and shallow compared to the other two levels of \emph{Text Granularity}.}

% \subsection{\added{Coping "Bad" Conditions--Increasing Coding Conformity}}

% \subsubsection{Why the Baseline Condition was Perceived Worst?}
% \added{We mentioned in RQ3 (see section \ref{sec:rq3}), there were three conditions that are less helpful: \mi $\times$ \sele, \mi $\times$ \sent, and \sh $\times$ \para, and even worse, the baseline condition \mi $\times$ \sele engenders the least \he. 
% As we analysed in section \ref{sec:codingbehavior:sent=sele}, users show similar \cb (e.g., number of selections, length of selections) and \sr in \sent and \sele.
% The observation in \suggestionQuality also showed no much difference between them.
% Thus, the two less helpful conditions \mi $\times$ \sele, \mi $\times$ \sent "should" be expected as similar. 
% However, when looking at their \he and \suggestionQuality, \textbf{we surprisingly found contradicting comparisons: \mi $\times$ \sent engenders more \he than \mi $\times$ \sele.}
% One explanation could be with \mi, long codes and short codes were mixed in the code suggestion list, while it was good because of 32\% \sr, making it hard for users to find useful information to select or refer to. The additional flexibility, especially in \sele codes, while potentially positive for the users, seems to negatively impact the user’s \he with the suggestions.}

%\subsubsection{How "Bad" Conditions can be Converted to "Good"?--Increase Conformity}
% \label{sec:disc:choose-or-refer}
% \added{Interestingly, in both above cases, if we forced users to code with \sh or \lo, their perceived trust becomes very high. This change allows users to do coding using a highly conforming way, allows them to predict the output of the system stably.
% As such, the system can perceived as helpful by 1) providing stable and relevant information that cannot choose but can refer to, or 2) providing relevant information that can directly choose. \textbf{Both situations show that the system can be "expected" and "relied on" properly}, making people feel more helpful than a system that either cannot choose or cannot refer (\mi $\times$ \sele), \textbf{contributing to the build of another construct of trust--perceived trustworthiness \cite{vereschak2021evaluate}.}}



% \subsection{\added{Does Increased Conformity Always Work? Coping "Difficult" Coding Tasks}}
% \label{sec:disc:difficulty}
% \added{We noticed that we should avoid using \sh when applying \opencoding for \para as this task is hard for both system and the user: 
% 1) The difficulty here for the system is to provide a relevant \sh label.
% If a system always has a low chance to make connections between the suggestions (see Figure \ref{fig:topk}) and their own codes/selections on a hard task (see the highest decision time for \para in Figure \ref{fig:decision_time}) in a limited time and selection (implying by the time = decision time $\times$ a number of selections, see Figure \ref{fig:decision_time} and Table \ref{tab:outcome}), and as such, the suggestion quality is likely degraded, leading to lower levels of trust. 
% 2) if a human needs to summarize for a long paragraph, their decision time will be significantly increased (up to 40\%). When discussing with participants, they reported that the \para tasks were deemed as the hardest, as it is harder to find a label for a code that fits an entire paragraph as opposed to a shorter textual unit (\sele or \sent). 
% The chance of reusing previous codes inevitably decreased, which can be reflected in the system's performance \suggestionQuality(see section \ref{sec:RQ:code-relevance}).
% This implies that \textbf{the task difficulty and limited interaction between the system and humans also limits the building of trust and helpfulness.} Thus it is better that the system takes this chance to show more ability and enable people to get more helpfulness from outside, e.g., self-generate codes, do text summarization, and connect to theory.
% }

% \gao{LS: little chance to match with each other => very hard task; LP: higher chance to match with each other; LE: }


% % \subsection{But Perceived Trust is High with Harder Tasks}
% \subsubsection{How to Get Build Better Trust on Difficult Tasks?}
% \added{In our case, if \sh is substituted as \lo or \mi, which shows similar \cb (length and number of selections, codes), it becomes better in both system's \suggestionQuality, \cq and \he
% while we noted that the \sr was the lowest for \para settings overall. 
% The subjective feedback showed that for \lo conditions, users seems to be positive that were able to work from these longer codes.
% As we mentioned in section \ref{sec:disc:choose-or-refer}, either choosing or referring assistance can help users to build trust.
% In fact, when performing the \para tasks, users would check and refer to all the suggestions provided by the AI, and while they reported that the suggestions were individually not fully relevant enough to be selected (hence the low \sr), they would still be able to use them as references for their new codes, or first select the codes and then edit the close code suggestion to their desired codes (i.e., delete irrelevant words, keep or change part of the words). This is validated in the user's subject preferences (RQ3). \gao{replace RQ3 after reordering}. In addition, \lo also showed to users that the system can grasp the main idea of the text selected, while \sh only provided limited information in the code suggestions provided by the system. }
% Moreover, our observations on \pt for harder tasks, also suggests that the trust we measured depends on users' expectation. In situations where the tasks gets significantly harder to perform, users will appreciate any help, even if not very accurate. 
% % As such, our AI system was useful for users for both simple (\sele and \sent) and hard (\para) tasks regardless its accuracy which sheds new light into how AI can be used for qualitative coding. 

% % \subsection{Behavior Trust is High with Better Suggestions}
% \subsection{\added{Coping Over-reliance and Low Diversity Problem}}
% When looking at \emph{Text Granularity}, our results show that for simpler tasks (i.e.  at \sele and \sent levels), \bt is higher, as users tend to use the suggestions more: users selected a suggestion more than 26\% for \sele and \sent, in contrast to 16\% in the \para conditions. \added{The high variance we observed also suggests that some participants may have relied on the AI system in those conditions. 
% One the one hand, this is still a positive thing, as a lower number of unique codes actually improves the conformity, decreases the outliers, and thus decreases the difficulty of classification for later tasks. It can also be seen as slightly negative, depending on the phase of the coding process: in early exploration phases, diversity is quite important for users to form and evolve the final codebook. 
% On the other hand, if the user always reuses the past codes (hence few new codes are created), this will let them rely on the system too much and thus decrease their motivation or chances to provide diverse expressions. While our motivation is to improve system's reliability to better assist users' qualitative coding, it is never good to overlook the potential risk of over-reliance and low-quality results (high \sr but low diversity).} 

% \subsubsection{How to Ease Over-reliance Problem?}
% \added{To tackle this problem, if we force users to add longer codes, the increased length of codes helps users stay longer on the text than before (see Figure \ref{fig:decision_time}), helping them do more reflections, and also the increased time forces them to generate more qualified and diverse codes than before (see Figure \ref{tab:codequality}), making them feel those code suggestions, which were seeding from their own code history, have higher perceived helpfulness (see Figure \ref{fig:helpfulness}), with only a little cost of decreased \sr overall. 
% Also, long codes could contains multiple short codes, enforcing users increase their code diversity, having higher ability to be seen as "relevant" to users' final codes, and thus providing higher "reference" assistance.
% In addition, \sele and \sent can be seen have similar behaviors in terms of \cb (number and length of selections) when using \sh. By applying \sent, users are forced to check all details in a specific way, thus generating more unique codes, with a good \sr (see Figure \ref{fig:selecting}).}

% \gao{comparison1: the lowest selecting rate but the highest code suggestion quality in RQ1—-model comparison2: the highest selecting rate but the very low code suggestion quality in RQ1—–model}



% Participants reported that the suggestions were less relevant on \para tasks, based both on the reduced data used for training and length of text which makes it hard to summarize a paragraph. 
% This issue of creating a suitable code is even stronger in the \sh $\times$ \para conditions which yields the lowest \sr for suggestions. 

% So it is fair to assume that users will display a higher level of trust with better suggestions.
% \simon{<< Discuss code quality as well \gao{[fixed]} >>}
% % 
% \simon{<<Managing Trust Expectations and Usefulness of AI>> From our experiment, and given the differences in terms of \bt and \pt we observed, we understand that trust is a complex notion. Previous literature highlighted that trust is correlated with accuracy (or the quality of the suggestions) \cite{papenmeier2022s, yin2019understanding}. Our results confirm this general trend: \bt (through \sr) was generally higher in conditions with better suggestions (\sele and \sent). \gao{[fixed, added into above]}}


% \simon{<<Reliance on the System>><<What is over-reliance? what is low reliance?>> <<Code Quality and Trust>> <<Short summary:  sentence>> selective, which confirms the general trend. The case of paragraph which was already discussed as well. \gao{[fixed]}}



